BumbleBee: Application-aware adaptation for container orchestration

Modern applications have embraced separation of concerns as a first-order organizing principle through the use of containers, container orchestration, and service meshes. However, adaptation to unexpected network variation has not followed suit. We present BumbleBee, a lightweight extension to the container ecosystem that supports application-aware adaptation. BumbleBee provides a simple abstraction for making decisions about network data using application semantics. Because this abstraction is placed within the communications framework of a modern service mesh, it is closer to the point at which changes are detected, providing more responsive and effective adaptation than possible at endpoints.

==> text/api.tex <==

\subsection{\name{'s} API}

\system views the world from the perspective of a single pod and how that pod wants to react to changes in the network. \system exposes the abstraction of a single \textit{mutable} queue for each route (source-destination pair) in a pod, where developers can access and modify each queue.




\system{} aims to provide an interface that is both \textit{simple} and \textit{low-overhead} (Section \ref{sec:principles}). This motivated a few key design decisions. We first
explored declarative interfaces like YAML or SQL, but decided it had too much unnecessary functionality that could be a runtime
liability, while simple things were too complicated to express. 
In addition, nearly all adaptation strategies of which we are aware are implemented in imperative languages. Giving \system a declarative interface would have not only asked developers to reimplement their strategies in a new language, but it would also have asked them to re-conceptualize those strategies in an unfamiliar style. 
Thus, we shifted from
a declarative SQL/YAML interface to imperative Lua scripting environment.
\footnote{Envoy recently announced support for running WebAssembly in filters, which could potentially allow \system to support any high-level language that compiles into WebAssembly bytecodes (in addition to Lua). We leave this for future work.}

Furthermore, we explicitly do not support the use of Lua libraries beyond the standard, built-in set, keeping in-script behavior simple, low overhead, and less prone to security attacks. We support the use of such complicated functionality through asynchronous external calls.




\subsubsection{Common adaptation strategies} 

We considered a variety of case studies in
which adaptation in the network might be helpful. The cases studied span across various domains (listed below). %including video analytics, video streaming, IoT networks, stream processing frameworks and geo-distributed storage systems.
While on the surface they look different, we discovered the common adaptation strategies in all these domains follow \textit{four main patterns: transform, re-order, redirect, or drop}.


%\noindent\textbf{Adaptation case studies;}

\squishlist
	\item \textit{Video analytics:} where machine learning (ML) is used on a continuous stream(s) of video frames and uploading all the raw frames with desired latency is not feasible. Possible adaptations could include 
	reducing resolution of data (transform)~\cite{Pakha18}, e.g., with a ML model not very sensitive to resolution;
	dropping frames (drop)~\cite{hsu2019couper}, e.g., when running object detection on slow changing feed;
	redirecting data to a cheaper model on the edge (redirect)~\cite{hsieh-osdi18, jiang-sigcom18}, e.g., for filtering data or in face of disconnections;  
	%%%%%%%%%%%
	\item \textit{Video streaming:} where live or on-demand movies are streamed from a server to a client. Possible adaptations could include: 
	reducing resolution of frames (transform)~\cite{yan-nsdi20, mao-sigocmm17}, 
	reducing frames-per-second (transform and drop)~\cite{Wang05},
	%%%%%%%%%%
	\item \textit{Video conferencing:} where two or more clients are interactively talking via video call. Possible adaptation strategies include: 
	reducing resolution of calls (transform)~\cite{De08, Zhang12}, %% skype
	\todo{downgrading to voice call (transform)}, %% facetime does this, couldn't find paper reference.
	\todo{skipping part of the conversation if delayed too long (drop)}, %% ughhhh couldn't find reference.
	and for mobile users using a different meet-up server (redirect)~\cite{Jiang16}.
	%%%%%%%%%%
	\item \textit{IoT networks} collecting and processing sensor data from 100s or 1000s of sensors. Possible adaptation strategies include: 
	filtering data below a threshold (drop)~\cite{Greenstein06}, %% lmao, Ben's
	aggregating data in averages or histograms (transform)~\cite{Jang16} %% Mine!
	while also placing raw sensor data at the tail of the queue for background uploading (re-order)~\cite{Higgins10}. %% Brett & Jason's
	%%%%%%%%%%
	\item \textit{Stream processing frameworks:} processing massive streams of data in a distributed framework for real-time insights such as anomaly detection. Possible adaptation strategies include: 
  filtering of low-importance messages (drop)~\cite{Tatbul03}, 
	aggregating/reducing multiple messages into one (transform and drop)~\cite{Tatbul06},
	reordering new messages over backlogged ones that have passed their deadline (re-order)~\cite{Avnur00, Raman99},
	moving messages assigned to an overloaded worker to other workers (redirect)~\cite{Cherniack03}.
	%%%%%%%%%%
	\item \textit{Geo-distributed storage systems:} storing and reading data across multiple geo-distributed locations. Possible adaptation strategies include: 
	prioritizing new writes over old writes upon reconnection (re-order), %% Coda? 
	\todo{compacting writes by deleting ones that override old values (drop)}, 
	redirecting writes to another location that is currently connected (re-direct)~\cite{Bogdanov18},
	\todo{lossy compression of data especially large blobs (transform)} %% this one is too obvious for citation
	%%%%%%%%%%
	
\squishend


%Based on the adaptation strategies in all these domains,  we identified \textit{four main patterns: transform, re-order, redirect, or drop
%	application data}. 
%This led to a core design decision:\system only needed to work on a
%contiguous range at the head of the data queue; there was no compelling need for arbitrary
%queue access. 


\begin{figure}[t]
  \begin{lstlisting}[style=lua,xleftmargin=13pt]
  function envoy_on_request(h)
    -- for each sink
    for queue in h:Queues():getQueue() do
      -- check the route
      route = queue:route()
      if string.find(route, "cloud") then
        -- check current bandwidth estimate
        bw = queue:getBW()
        if bw == 0 then
          -- if disconnected
          -- redirect the request to the edge
          h:redirect("edge-detector")
        elseif bw < required then
          -- if bw is too low
          -- transform the request to lower-res
          h:transform("180p")
        end
        if bw < required/2 then
          -- if bw drops well below required
          -- notify the request source
          h:notify(bw)
        end
      end end end
	\end{lstlisting}
	\caption{This simple Lua script for the traffic-monitoring application redirects requests to the edge when the network becomes disconnected, down-samples enqueued requests when bandwidth drops, and invokes a registered callback network conditions change significantly.} 
	\label{lst:yolo}
\end{figure}

This study also led to a core design decision:\textit{\system only needed to work on a
	contiguous range at the head of the data queue}; there was no compelling need for arbitrary
queue access.

\joseph{feel disjoint to jump into queue abstraction discussion (and the
abstraction has not been discussed clearly so far). What about we do this:
move video analytics to the last, 
move any discussion about patterns (in 4.1.1) to very last so that we begin to
bring reviewers to queue abstraction, like ``based on variety of adaptation
strategies already in-use, we identify four patterns that can be easily
supported with a \emph{message queue} abstraction.''
, and then we show here is a script snippet. I prefer moving detailed script
explanation in eval section. Here, we can simply say the script is simple but
supports custom adaptation logics, thanks to queue abstraction.}


What about we move video
analytics to the last

\noindent\textbf{\system{} Lua script interface:}
Listing ~\ref{lst:yolo} shows a sample \system{} adaptation logic for a traffic monitoring application.
\shadi{should we expand on the example?}
The main abstraction exported to \system scripts is a message queue. Each script can iterate queues maintained by the queue manager (Line 3). These methods allow a script to access queue properties, such as its length, route, or observed bandwidth (Line 5--8). 
The queue iterators are also used to apply in place transformations, such as redirecting messages to another endpoint (Line 12), as well as external callbacks (further detail in Section \ref{sec:callback}) such as transforming the message (Line 16) or notifying the application (Line 21). 
 Other adaptation strategies such as dropping all messages, dropping the head of the queue, and reversing the queue's order are implemented in a similar fashion.



 \noindent\textbf{Metrics exposed:}
 To help scripts make good adaptation decisions, \system exports a number of runtime performance metrics. At the lowest level, \system exposes TCP metrics, such as the congestion window size, number of in-flight packets, and mean round trip time (RTT). \system also exposes the average end-to-end latency for messages in a queue, which Envoy calculates using request and response arrival times. In addition, \system provides information about how long each messages has spent in a queue through an object-item's age property. 
 
 Finally, network bandwidth is a crucial metric for numerous adaptation strategies.  \system does not give scripts information about the available bandwidth along a physical link, but it calculates the observed bandwidth for messages forwarded from particular queue. This allows scripts to reason about the observed bandwidth along their path of interest. For example, scripts can detect that a path has been disconnected if its observed bandwidth drops to zero.
 \shadi{@joseph: are we missing anything?}
 
 Table~\ref{tab:bb_api} summarizes \system's in-network scripting interface and the metrics exposed.
 


==> text/background.tex <==
\section{Background}
\label{sec:background}

%\system is an in-networking processing framework that executes arbitrary user-defined adaptation logic.
\system depends on three enabling technologies. The first is container orchestration 

The remainder of the section describes 

\noindent\textbf{Container orchestration platform:} These platforms automate the deployment, scaling, and
management of containerized applications. Developers simply define a manifest
of how their application deployment should look like, e.g., how many
containers to have, what container image to use, what ports to expose, etc.
The orchestration platform automatically deploys this manifest while ensuring other functionalists including failure recovery,
load-balancing, auto-scaling, etc. 

\system use Kubernetes \cite{hightower-oreilly17}, the most widely used platform, as its base orchestration platform. 
In Kubernetes, a `pod' is the smallest unit of deployment, similar to a process
in operating systems. A pod encapsulates one or more containers that share
underlying resources, like threads. Typically, an application deployment
consists of one or more pods. %, as shown in Figure~\ref{fig:envoy}. %\ref{fig:service-mesh}.

\begin{figure}[]
	\centering
	\includegraphics[width=\columnwidth]{figs/envoy.pdf}
	\caption{Envoy's Architecture in a single pod.}
	\label{fig:envoy}
\end{figure}

\subsection{Container orchestration}



\subsection{Sidecar proxies}

\noindent\textbf{Envoy:} Envoy intercepts communications in containerized platforms like Kubernetes~\cite{envoy}. In every application pod, Envoy injects a sidecar proxy as shown in Figure~\ref{fig:envoy}. This proxy intercepts all network packets to/from the application containers by loading {\tt iptable} rules at startup time.
Inside Envoy, these redirected messages go through a chain of pre-configured \emph{filters}. Filters have full control over messages and can perform various operations on them, such as redirecting to another destination, dropping messages, or transforming the payload. Envoy works fully transparently, without the need for any application modification (unlike many prior systems~\cite{noble-sosp97, fox-asplos96}).  \system is implemented as part of Envoy.




%\begin{figure}[]
%	\centering
%	\includegraphics[width=\columnwidth]{figs/service-mesh.png}
%	\caption{Kubernetes pods and service meshes. 
%    \joseph{Do we really need a diagram?} \shadi{I think it helps to clarify the service mesh. If we are short on space we can remove it.}
%  }
%	\label{fig:service-mesh}
%\end{figure}
%
%\noindent \textbf{Service mesh:} A service mesh is an architectural design to manage communication among containerized \textit{services}. A service is a logical set of pods
%designed to achieve singular functionality, e.g., a database
%service consists of pods that handle queries. Services simplify the development and management of applications by dividing the applications into independent components, so called a ``microservice'' architecture. At the same time, microservices introduce complexities in connecting the various services, e.g., load balancing, authentication, etc.
%Service meshes~\cite{istio, linkerd} hide these complexities by acting as a transparent layer managing communication between pods (within and/or across services).  A service mesh controls all ingress/egress traffic between pods by injecting a sidecar proxy container in each pod, as shown in Figure~\ref{fig:service-mesh}. The mesh provides insights and operational control on the communication, such as rate-limiting, A/B testing, and load balancing. Users can also define their custom processing logic.
%\system leverages this feature to execute arbitrary user-defined adaptations in the service mesh.
% 
 



% A service mesh~\cite{istio, linkerd} is an
%architectural design to manage communication among containerized applications
%so-called {\it microservices}. A microservice is a logical set of pods
%designed to achieve singular functionality. For example, a database
%microservice is consisted of pods that handle queries, retrieve data from
%storage, and record logs. In a monolithic design, one pod executes all
%operations; in distributed service mesh design, each pod is responsible for a
%subset of operations. The distributed nature of a service mesh achieves a
%great degree of fault-tolerance, scalability, and load-balancing by
%orchestrating traffics among pods. A service mesh controls ingress/egress
%traffic between pods by injecting a sidecar proxy container in pods (brown
%arrows and boxes in Figure~\ref{fig:service-mesh}). We revisit details of the
%sidecar proxy later in Section~\ref{sec:impl}.


% Commonly, applications are divided into independent \textit{services}, i.e., a
% logical set of pods performing one operation (e.g., a webserver service and a
% database service). This architecture is so called a ``microservice''
% architecture and it simplifies management, scaling, and programming of
% applications. However a microservice architecture, introduces complexities on
% connecting the various services, e.g., load balancing, authentication, etc.
% Service Meshes, such as Istio and Linkerd \shadi{cite}, have been developed to
% hide these complexities. The mesh is a configurable, low-latency, and
% transparent processing layer that manages communication between services. The
% mesh provides insights and operational control on the communication. A few
% examples include metrics and monitoring, rate-limiting, access control, A/B
% testing, and load balancing. Users can also define their custom processing
% logic.

% In a service mesh architecture, a sidecar proxy container runs alongside a pod
% (Figure \ref{fig:service-mesh}). Similar to other containers in a pod, the
% sidecar proxy is also managed by the orchestration framework (Kubernetes in
% our case). This proxy captures all the traffic to/from containers in that pod
% and routes their traffic accordingly to either: another sidecar proxy (mesh
% traffic), a container in that pod (ingress traffic), or outside the cluster
% (egress traffic). 

% We have implemented \system on top of Kubernetes due to its widespread
% popularity. However, \system can work with any orchestration framework that
% can support a service mesh (described below). 


==> text/design-removed.tex <==

\subsection{\system{'s} abstraction motivation}

%To support the application-aware adaptation in network, we first study
%applications that already adapt to network changes internally. The study
%provides valuable lessons for designing \system with operations to support and
%a right abstraction to expose to the in-network script. The study spans across
%various domains, ranging from video streaming to geo-distributed storage
%applications. We discuss them turn by turn.

We studied
applications that already adapt to network changes across various domains, ranging from video streaming to storage
applications.
 While on the surface the applications in each category adapt differently, we realized they follow four common patterns: \emph{transform}, \emph{drop},
\emph{redirect}, and \emph{re-order}, as described in more detail below. 


\squishlist
	%%%%%%%%%%%
	% \item \textit{Video streaming:} where live or on-demand movies are streamed from a server to a client. Possible adaptations could include: 
  % Possible adaptations could include: 
  % reducing resolution of frames (transform)~\cite{yan-nsdi20, mao-sigocmm17}, 
  % reducing frames-per-second (transform and drop)~\cite{Wang05},
\item \textit{Video streaming:} live or on-demand videos are streamed from a
  server to a client. When bandwidth is constrained, parties involved 
  \emph{transform} streams to lower video resolution, 
  or \emph{drop} frames-per-second~\cite{Wang05}.
\joseph{how is video streaming different from video conferencing?}

	%%%%%%%%%%
	% \item \textit{Video conferencing:} where two or more clients are interactively talking via video call. Possible adaptation strategies include: 
	% reducing resolution of calls (transform)~\cite{De08, Zhang12}, %% skype
	% \todo{downgrading to voice call (transform)}, %% facetime does this, couldn't find paper reference.
	% \todo{skipping part of the conversation if delayed too long (drop)}, %% ughhhh couldn't find reference.
	% and for mobile users using a different meet-up server (redirect)~\cite{Jiang16}.
\item \textit{Video conferencing:} multiple users interactively video-chat.
  When network is congested, clients \emph{transform} frames to lower
  resolutions~\cite{De08, Zhang12}, or \emph{drop} to voice-only mode (e.g., FaceTime ``poor connection''~\cite{Robinson16}). For
  consistent poor network conditions, they \emph{redirect} to calls through a
  different meet-up server~\cite{Jiang16}, or occasionally \emph{drop} out-of-sync frames if delayed too long.

 	%%%%%%%%%%
	% \item \textit{IoT networks} collecting and processing sensor data from 100s or 1000s of sensors. Possible adaptation strategies include: 
	% filtering data below a threshold (drop)~\cite{Greenstein06}, %% lmao, Ben's
	% aggregating data in averages or histograms (transform)~\cite{Jang16} %% Mine!
	% while also placing raw sensor data at the tail of the queue for background uploading (re-order)~\cite{Higgins10}. %% Brett & Jason's
\item \textit{Internet of Things (IoT):} distributed clients collect and
  stream sensor data to the cloud. The clients react to changes in network
  environment by dropping (filtering) data points below a
  threshold~\cite{Greenstein06}, aggregating or \emph{tranforming} data into
  an average or histogram~\cite{Jang16}, and \emph{re-ordering} low-priority
  data points to the tail of the queue~\cite{Higgins10}.

	%%%%%%%%%%
	% \item \textit{Stream processing frameworks:} processing massive streams of data in a distributed framework for real-time insights such as anomaly detection. Possible adaptation strategies include: 
  % filtering of low-importance messages (drop)~\cite{Tatbul03}, 
	% aggregating/reducing multiple messages into one (transform and drop)~\cite{Tatbul06},
	% reordering new messages over backlogged ones that have passed their deadline (re-order)~\cite{Avnur00, Raman99},
	% moving messages assigned to an overloaded worker to other workers (redirect)~\cite{Cherniack03}.
\item \textit{Stream-processing applications:} distributed workers process
  \emph{continuous} streams of data for real-time insights (e.g., fraud
  detection). However, the distributed nature of the jobs often encounter
  turbulent network environment. The applications adapt by \emph{dropping}
  less important messages~\cite{Tatbul03}, \emph{re-ordering} new messages to
  the front queue to avoid backlogs~\cite{Avnur00, Raman99},
  \emph{transforming} multiple messages to aggregated message~\cite{Tatbul06},
  and \emph{redirecting} messages that are assigned to overloaded worker to
  other workers~\cite{Cherniack03}.

	%%%%%%%%%%
	% \item \textit{Geo-distributed storage systems:} storing and reading data across multiple geo-distributed locations. Possible adaptation strategies include: 
	% prioritizing new writes over old writes upon reconnection (re-order), %% Coda? 
	% \todo{compacting writes by deleting ones that override old values (drop)}, 
	% redirecting writes to another location that is currently connected (re-direct)~\cite{Bogdanov18},
	% \todo{lossy compression of data especially large blobs (transform)} %% this one is too obvious for citation
\item \textit{Geo-distributed storage systems:} systems read and write data
  stored across multiple geo-distributed locations. When latency is high,
  systems \emph{redirect} writes to another location~\cite{Bogdanov18,
  Uluyol20}.
% prioritizing new writes over old writes upon reconnection (re-order), %% Coda? 
% compacting writes by deleting ones that override old values (drop), 
%% Need to ask Brian and Landon for whether above two violate consistency.
% lossy compression of data especially large blobs (transform) %% This is not adaptive

	%%%%%%%%%%
% \item \textit{Video analytics:} where machine learning (ML) is used on a
%   continuous stream(s) of video frames and uploading all the raw frames with
%   desired latency is not feasible. Possible adaptations could include reducing
%   resolution of data (transform)~\cite{Pakha18}, e.g., with a ML model not
%   very sensitive to resolution; dropping frames (drop)~\cite{hsu2019couper},
%   e.g., when running object detection on slow changing feed; redirecting data
%   to a cheaper model on the edge (redirect)~\cite{hsieh-osdi18,
%   jiang-sigcom18}, e.g., for filtering data or in face of disconnections;  

\item \textit{Live video analytics:} machine learning (ML) is used on a
  continuous streams of video frames. When bandwidth is insufficient to upload
  all the raw frames with desired latency, the applications 
  \emph{transform} frames to lower resolutions~\cite{Pakha18}, or
  \emph{drop} intermediate frames for motionary videos~\cite{hsu2019couper}.
  For disconnections, they \emph{redirect} to a cheaper ML model on the
  edge~\cite{hsieh-osdi18, jiang-sigcom18} that provides less accurate results
  than an resource-expensive model in the cloud.
\squishend


% While on the surface they look different, we discovered the common adaptation strategies in all these domains follow \textit{four main patterns: transform, re-order, redirect, or drop}.
%Based on the adaptation strategies in all these domains,  we identified \textit{four main patterns: transform, re-order, redirect, or drop
%	application data}. 
%This led to a core design decision:\system only needed to work on a
%contiguous range at the head of the data queue; there was no compelling need for arbitrary
%queue access. 
%{\color{blue}
%At the first glance, applications in each category adapt differently; we
%find that complex adaptation logics can be supported with a common set of
%primitive adaptation operations: \emph{transform}, \emph{drop},
%\emph{redirect}, and \emph{re-order}. 
%This led to a core design decision:\system only needed to work on a contiguous
%range at the head of the data queue; there was no compelling need for
%arbitrary queue access. 
%}

Moreover, we realized that \textit{adaptation strategies only needed to work on a contiguous
range at the head of the data queue;} there was no compelling need for
arbitrary data access. Thus, \system{} exposes the abstraction of a single \textit{mutable} queue for each
route (source-destination pair) to the adaptation scripts.

%
%{\color{red}
%This leads us to expose a single mutable queue abstraction to the in-network
%script.
%\system exposes the abstraction of a single \textit{mutable} queue for each
%route (source-destination pair) in a pod, where developers can access and
%modify each queue.
%}


==> text/design.tex <==
\section{Design and Implementation}
\label{sec:design}

 \begin{figure}[]
	\centering
	\includegraphics[width=\columnwidth]{figs/k8-deployment.pdf}
	\caption{Kubernetes deployment of a distributed application with \name{} enabled.
}
	\label{fig:k8-deployment}
\end{figure}

\shadi{high level comment: the flow of the paper seems a bit broken. the transition form one section to another is a bit abrupt}

\shadiC{
\system{} is implemented as an Envoy filter, wherein all application traffic goes through Envoy and therefore through the \system filter.
We use Istio to
deploy \system-enabled applications pods in a Kubernetes cluster.
Figure~\ref{fig:k8-deployment} illustrates overall steps involved. Users
define their application container images and their corresponding configurations in a YAML manifest.
When deploying to a Kubernetes cluster, Istio automatically injects Envoy
sidecar containers in the application pods. In addition, users define their adaptation logic as a simple Lua script. This adaptation logic is deployed through Istio in the \system{} filter where \system automatically invokes any user-defined adaptation logic when necessary. The adaptation logic acts as an modifiable configuration file that users can easily change on-the-fly without stopping or redeploying their application.
}

\input{text/api}
\input{text/api-table.tex}

\subsection{\system{} Architecture}
\begin{figure}[]
	\centering
	\includegraphics[width=\columnwidth]{figs/envoy-BB.pdf}
	\caption{{\name} extends the Envoy sidecar (\name{} components marked as yellow).}
	\label{fig:envoy-with-BB}
\end{figure}

Figure~\ref{fig:envoy-with-BB} shows a high-level overview of \system{} and
how the user-defined adaptation logic is deployed and executed upon in the \system{} filter. This rest
of this section describes the three key components of our \system design
choices: a queue manager that maintains message queues, an in-network scripting facility that executes custom application logic as messages arrive, and a callback mechanism that allows scripts to interact with other parts of an application. 

% \shadiC{
	
% \system is implemented as part of Envoy. Our current implementation uses Istio for deployment, but it is service-mesh agnostic. Figure~\ref{fig:k8-deployment} shows the overall deployment of containerized application with \name{} enabled. Users develop their container images and configuration manifest (as done traditionally) alongside a simple and decoupled adaptation logic. Using Kubernetes and Istio, the application pods are injected with Envoy sidecars and deployed to the cluster. Then, \name{} uses the adaptation logic written by the user to automatically trigger adaptation when required.

% \system is implemented as Envoy filter. 
% Figure~\ref{fig:envoy-with-BB} shows a high-level overview of \system{} and how the user-defined adaptation logic is deployed and executed upon. This rest of this section describes the three key components of our \system design: a queue manager that maintains message queues, an in-network scripting facility that executes custom application logic as messages arrive, and a callback mechanism that allows scripts to interact with other parts of an application. 



% }



\subsubsection{Queue manager}

%This approach is well suited to Envoy's stateless, per-message filters, but \system's core abstraction is a shared message queue.

\shadiC{
Envoy's stateless, per-message filters abstraction is well-suited for common functionalities provided by service meshes (load balancing, filtering, etc.), but \system's core abstraction is a stateful shared message queue.
}
So, \system extends Envoy with a separate queue-manager that runs
concurrently with the worker threads. Worker threads pass messages to the
queue-manager through the \system filter. The \system filter buffers data
until a complete network message (e.g., HTTP request/response,
Netty~\cite{netty} message) has been assembled, and then forwards the message
to the queue manager. 
\joseph{Should we say network message or protocol message? Not sure which one
is a correct terminology here}

The queue manager manages pairs of message queues (one for requests and one responses) and threads (one for each queue), and exposes a small number of methods that can be invoked by \system filter instances within worker threads. The queue manager creates a default pair of queues and threads, but applications can instruct the manager to create a pair of queues and threads to handle communication for pods with specific names. For example, in its orchestration configuration an application may name pods containing an object-detector running on the cloud "cloud-object-detector.local." It can then instruct \system to create queues in each pod's Envoy for handling requests to those pods. When a \system filter passes a message to the queue manager, the manager adds the message to the queue created to handle the message's destination (for outgoing messages) or source (for incoming messages). 
\shadiC{We use a simple, per-queue locking scheme to synchronize access to all queue-related state. 
	Moreover, to give scripts access to an underlying queue, \system uses Envoy macros to export a handful of C++ methods from the queue manager to the Lua runtime.}

The queue manager's thread pairs are primarily timer handlers that implement a token-bucket algorithm. On wakeup, a queue-manager thread checks its bucket to determine whether it has enough tokens to forward the head of its queue via Envoy's event dispatcher. The queue manager avoids spurious wakeups in two ways. First, when a queue is empty, its thread will block on a condition variable instead of polling. After a worker thread adds a new message to a queue, it signals the queue's condition variable. Second, when a queue is not empty, its thread sets its timer to wakeup when it will have enough tokens to forward the head of the queue. In our current implementation, the minimum sleep time is 1\unit{ms}.

%\shadi{do you cover that part of the queue is unmodifiable?}
%\shadi{when running a script on the queue, does the rest of the system proceed or is this a blocking action?}



%\begin{table*}[]
%	\begin{tabular}{|p{0.05 \linewidth}|p{0.4 \linewidth}|p{0.15 \linewidth}|p{0.2 \linewidth}|p{0.07 \linewidth}|}
%		%			|p|p|p|p|p|}
%		domain          & Sample applictions                                                                                                                       & adaptation                      & why?                                                     & category  \\ \hline
%		Video analytics & machine learning is used on a continuous stream(s) of video frames and uploading all the raw frames with desired latency is not feasible & reduce resolution of each frame & machine learning model not  very sensitive to resolution & transform  \\  \hline
%		&                                                                                                                                          &                                 &                                                          &           \\
%		&                                                                                                                                          &                                 &                                                          &          
%	\end{tabular}
%\end{table*}

\subsubsection{In-network scripting}



\shadiC{
The \system filter and queue manager push and pop from shared queues, but \system needs to apply custom adaptation logic to the shared queues. When a worker thread loads a \system filter, the filter reads the appropriate script from the orchestration configuration and launches it within a Lua runtime, a feature natively supported by Envoy. 
}
 

%The \system filter and queue manager push and pop from shared queues, but \system applications need more ways to interact with messages. Fortunately, Envoy supports Lua scripting within filters, and \system leverages this feature to support application-aware adaptation. Similar to how a \system application creates custom message queues through its orchestration configuration, an application can also associate short Lua scripts with those queues. When a worker thread loads a \system filter, the filter reads the appropriate script from the orchestration configuration and launches it within a Lua runtime. 


%We also considered declarative interfaces like YAML or SQL for in-network adaptation. However, we felt that an imperative approach would be easier for many developers, and Envoy's existing support for Lua made it easier to build a prototype. It is worth noting that Envoy recently announced support for running WebAssembly in filters, which could potentially allow \system to support any high-level language that compiles into WebAssembly bytecodes. We leave this for future work.

\system executes scripts \textit{when messages arrive} for a purely practical reason: Envoy already supports running Lua scripts in filters. The primary drawback of running scripts when messages arrive is that it ties adaptation frequency to message arrival rate. In the worst case when messages stop arriving, an application's adaptation scripts will also stop executing. This design decision may be worth revisiting, but in our limited experience with \system, linking adaptation frequency to arrival rate has not caused any problems
{\color{blue} (discussed later in Section~\ref{sec:limit}). }

%The main abstraction exported to \system scripts is a message queue. Each script can iterate queues maintained by the queue manager. To give scripts access to an underlying queue, \system uses Envoy macros to export a handful of C++ methods from the queue manager to the Lua runtime. These methods allow a script to access queue properties, such as its length, as well as apply coarse transformations such as dropping all messages, dropping the head of the queue, and reversing the queue's order. In addition to accessing a message queue, \system scripts can access queue-iterator and queue-item objects for traversing the queue and reasoning about individual messages, respectively. We use a simple, per-queue locking scheme to synchronize access to all queue-related state. 

%To help scripts make good adaptation decisions, \system exports a number of runtime performance metrics. At the lowest level, \system exposes TCP metrics, such as the congestion window size, number of in-flight packets, and mean round trip time (RTT). \system also exposes the average end-to-end latency for messages in a queue, which Envoy calculates using request and response arrival times. In addition, \system provides information about how long each messages has spent in a queue through an object-item's age property. 
%
%Finally, network bandwidth is a crucial metric for numerous adaptation strategies.  \system does not give scripts information about the available bandwidth along a physical link, but it calculates the observed bandwidth for messages forwarded from particular queue. This allows scripts to reason about the observed bandwidth along their path of interest. For example, scripts can detect that a path has been disconnected if its observed bandwidth drops to zero.

%%	\system is operating at the in-network level and
%	it can provide fine-grained  visibility in latency. Thus, it exposes two latency
%	metrics: i) end-to-end latency, as time difference between the request being
%	received and corresponding response being sent back and ii) message age,
%	as the time spent in \system's Queue.  


%\item \textbf{Bandwidth metrics:} \system exposes the rate (B/s) at which the queue is draining as the \textit{observed bandwidth} metric. This is what a particular queue is observing as its allocated bandwidth which may be different than the actual bandwidth of the physical link.
%\item \textbf{Size and length metric:} \system exposes several metrics including the \textit{queue length}, i.e, the number of messages enqueued in \system's queue, and the \textit{message size}, i.e., the size of each individual message.

\subsubsection{External callbacks}
\label{sec:callback}
\system's scripting environment allows applications to perform simple, local processing on enqueued messages. However, many applications can benefit from richer interactions between scripts and the rest of the application. For example, an application may want to use a script as an in-network watchpoint for changing conditions, such as notifying a pod when observed bandwidth falls below a threshold. This is useful for realtime video-analytics applications that reduce the resolution of video frames sent to an inference model when bandwidth drops. Or an application may want to transform message payloads in ways that are too complex for a lightweight Lua runtime. This is useful for video-streaming servers that want to downsample video chunks to prevent head-of-line blocking. To support this kind of functionality, \system allows scripts make two asynchronous callbacks to external endpoints on Envoy's async HTTP client thread. 

The simpler of the two is {\tt notify (metrics)}. An application's orchestration configuration can bind a list of RESTful endpoints to {\tt notify} invocations within a script. {\tt notify} takes a string as an argument, and when a script calls {\tt notify} the Lua runtime generates asynchronous HTTP calls with the string argument to any endpoints listed in the orchestration configuration.  \shadi{motivate the need for notify. It is breaking the separation of concerns argument.}

{\tt transform()} is a more complex callback. As with {\tt notify}, applications bind invocations of {\tt transform} to a RESTful endpoint through their orchestration configuration. When a script calls {\tt transform} on a queue entry, the Lua runtime marks the entry as "in progress" and asynchronously forwards the message payload to the registered endpoint. If a message moves to the front of the queue while marked in-progress, the queue-manager thread skips it, and sends the first entry not marked in-progress. When the endpoint returns with a transformed message payload, \system swaps in the new payload, updates the message header to reflect its new size, and remove its in-progress mark. 

In our experience, {\tt transform} is best used for complex computations that require specialized hardware, such as media transcoding. However, we believe that {\tt transform} could also prove useful in cases where a transformation requires access to state that is inaccessible to the \system filter, such as an external database. We are actively exploring such use cases.

%Table~\ref{tab:bb_api} summarizes \system's in-network scripting interface.

%Such notifications can be used by a video-analytics application that sends video frames from the edge to a machine-learning (ML) model in the cloud may want its camera to send lower resolution video when bandwidth to the cloud drops below a threshold. 

%For example, when network bandwidth drops, a video-streaming server may need to downsample high-resolution video chunks to prevent head-of-line blocking. 



%Both of examples show how applications can benefit from richer interactions between a \system script and the rest of the application. A watchpoint script for video-analytics could signal to a pod running on the camera when bandwidth changes. A video-streaming script could pass an enqueued video chunk to an external transcoder for downsampling when messages in front of it stall. 

%Developers register a callback by defining a \textit{callback reference} object that contains the list of endpoints to trigger a callback on. Developers can use this reference in their custom adaptation logic to trigger callbacks whenever needed. This is done by defining the trigger conditions and calling a {\tt notify (metrics)} function. This function also piggybacks a set of user-defined metrics with callback.


%This section discusses each of these in further detail.

%\system continuously monitors triggers defined for callbacks. When
%the conditions of callbacks are met, it automatically notifies the registered endpoints. It collects the values for the registered metrics and passes these with the callback notification. An example using the callback is shown in Figure \ref{lst:sample} Lines \shadi{XX}.


%% \subsection{Scripting API}

%% To hand messages to the queue manager, \system runs a custom Envoy filter that %% is based on Envoy's standard rate-limiting filter. Like \system, Envoy's %% rate-limiting filter needs to 

%% After messages go through {\name}'s filter, they are enqueued the queue manager %% until they are ready to be delivered. 
%% The queue manager dequeues messages and transfers them back to {\name}'s filter, %% which then the messages traverse the remaining filters registered in Envoy. The %% queue manager maintains a queue per destination pod plus an additional default %% queue for undefined destinations, e.g., outside the local cluster.

%% The queue manager also enforces a rate-limit per destination using a token-based %% approach to avoid bandwidth saturation by malicious applications. We currently %% support rate limiting in \unit{KB/s} granularity.

%% \system relies on the Envoy~\cite{envoy} sidecar to transparently interpose on %% network communication. 

%% we find that Envoy filter is stateless by its design choice. As a result, Envoy %% creates a filter thread per message, and destroys the thread when the message is %% dispatched, unlike a global TCP state shared with multiplexed connections (e.g., %% HTTP/2, WebSocket) over a full duty cycle. The stateless design imposes a %% challenge to expose a persistent message queue abstraction to the adaptation %% layer. 



%% Envoy executes each filter 




%% Inside Envoy, these redirected messages go through a chain of pre-configured . 

%% Envoy works fully transparently, without the need for any application %% modification (unlike many prior systems~\cite{noble-sosp97, fox-asplos96}), %% making it an ideal location to add {\name}'s adaptation. We implemented {\name} %% in Envoy by adding two components, a {\name} filter and queue manager, as shown %% in Figure \ref{fig:envoy-with-BB}. \shadi{add the flow for callbacks in Figure %% \ref{fig:envoy-with-BB}}.
%% We have implemented \system on top of Envoy v1.12 with $\approx$ 2900 lines of %% code (LOC).
%% We have modified Envoy for only 103 LOC to add features such as modifying %% headers by function pointer. 

%% Envoy proxies are -- it creates a filter thread per message which is destroyed %% after the message is dispatched. On the contrary, {\name} exposes a persistent %% and modifiable message queue abstraction, which requires state across messages. %% Therefore, {\name} includes 


%% %% queue manager

%% %% loading scripts

%% %% running scripts

%% %% queue abstraction

%% %% iterating over the queue

%% %% use 

%% \system is sits in the service mesh layer. It captures all messages going %% through and maintains a queue per each destination/flow. 
%% \system provides a simple interface for application developers to adapt both i) %% newly generated messages, and ii) prior on-the-fly messages waiting in the %% queue. 
%% \system exposes an array of low level networking metrics. Developers can write %% custom adaption logic that monitors their metrics of interests, and decides when %% and how to adapt. \shadi{add 1 sentence example}. 
%% Then, \system automatically and transparently, deploys the adaptation logic. It %% continuously monitors the predefined metrics of interest, and if any trigger an %% adaptation, it automatically applies the user defined adaptation logic.


%We discuss the metrics exposed and operations supported in \system in this section (as summerized in Table) in detail, turn by turn, in this section.


%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Metrics exposed by \system}
%\label{sec:design_metrics}

%\system operates at the in-network layer that gives it an enhanced
%visibility on low-level network metrics.
%\system exposes a rich set of these metrics to application developers, which they can use to specify
%conditions on which their custom adaptation logics should trigger. The
%following list contains a subset of these metrics: \shadi{@Joseph: are there other metrics we expose?}
%\begin{smitemize}
%	\item \textbf{TCP metrics:} \system exposes the low-level TCP metrics such as the congestion window size, number of in-flight packets, mean round trip time (RTT), delivery rate, etc. %These metrics are exposed both in a per message level (measured for each message) and per queue (aggregated metrics over the queue).
%	\item \textbf{Latency metrics:} 
%	\system exposes the average \textit{end-to-end latency} of messages in a queue. This is calculated as the time difference between the message being received by \system and the corresponding response being sent back. In addition, \system has fine-grained visibility into latency and it exposes the \textit{message age} metric as the time spent in \system's Queue
%%	\system is operating at the in-network level and
%	it can provide fine-grained  visibility in latency. Thus, it exposes two latency
%	metrics: i) end-to-end latency, as time difference between the request being
%	received and corresponding response being sent back and ii) message age,
%	as the time spent in \system's Queue.  
%	\item \textbf{Bandwidth metrics:} \system exposes the rate (B/s) at which the queue is draining as the \textit{observed bandwidth} metric. This is what a particular queue is observing as its allocated bandwidth which may be different than the actual bandwidth of the physical link.
%	\item \textbf{Size and length metric:} \system exposes several metrics including the \textit{queue length}, i.e, the number of messages enqueued in \system's queue, and the \textit{message size}, i.e., the size of each individual message.
	
%\end{smitemize}

%These metrics support cover a wide range of adaptation strategies. A few examples include detecting if congestion has increased (TCP metrics), an item has been waiting in the queue for too long (age), the bandwidth suddenly drops (observed bandwidth), or the queue is growing too large (queue length). New metrics can also easily be added to \system. 


%\subsection{Adapting messages}
%\label{sec:adapt-msg}


%One of the main differences of \system compared to prior works is the ability to modify outgoing messages that are still on-the-fly. When network conditions change abruptly, a large queue of outgoing messages may build up. After the connection recovers back to normal, the outstanding messages in the queue must drain first before any new incoming messages can be sent. As we show in our experiments (Section~\ref{sec:eval_fugu}), the ``head-of-line'' blocking issue can results in noticeable performance degradation. For example, a video streaming application may constantly experience high stall times (i.e., video being stalled), or an predictive maintenance application may not being able to send alerts in time. 

%Currently, when an application sends a message and the message enters the networking stack, it no longer has any control over that message. To bridge this gap, \system exposes a \textit{queue abstraction} to developers. This queue is a mutable queue of on-the-fly messages, which applications can access to adapt their prior messages. Applications have full control over this queue--they can iterate over the queue and modify, reorder, delete, or add any message in the queue. 


%\noindent\textbf{Programming Interface:}
%\system exposes an imperative adaptation interfaces in Lua scripting language. The use of imperative interfaces removes the need of platform-dependent implementations or interrupting services when
%rolling out new strategies. Also, developers have full flexibility on how to define their adaptation logic, as opposed to a declarative languages such as SQL. This adaptation logic is orthogonal to the application code itself and can be developed and modified independently. 

%\system provides access to both each individual messages content and headers (e.g., destination, payload size), and the global queue of messages (one queue per destination).
%The full list of APIs exposed by \system are shown in Table \ref{tab:bb_api}.
%Application developers register adaptation functions in form of Lua scripts. These functions are executed per message.




%\begin{figure}[t]
%\begin{lstlisting}[style=lua,xleftmargin=13pt]
%function adpat(h) --message handler h
%  cb = callback:register(endpoints)
%  for queue in h:Queues():getQueue() do
%    bw = queue:getBW()
%   ... 
%    -- 1. modify queue
%    if bw < required/2 then
%      for item in queue:getItem() do
%        if item:getAge() > deadline then  
%          item:drop()
%    ...
%    -- 2. adapt new data
%    elseif bw < required then
%      h:transform("180p")
%    ...
%    -- 3. use callbacks
%    if bw == 0  then
%      -- notify the callback handler
%      cb:notify(bw)
%    
%\end{lstlisting}
%\caption{Sample adaptation in \system with 1. adapting prior messages queued 2. adapting new incoming messages, and 3. using callback notifications} 
%\label{lst:sample}
%\end{figure}



%Figure \ref{lst:sample} shows a sample adaptation script in \system's interface. As shown, developers can identify their metric(s) of interest \shadi{Lines XX}, access the queued data, and define their custom adaptation logic and triggers \shadi{Lines XX}. 
%\system enables developers to modify messages arbitrarily. Specifically, they can i) reroute messages to a different destination (modifying the header), ii) transform the payload of a message as seemed fit (e.g., reducing the resolution of video frame or filtering some of the attributes), and iii) drop or insert the message. 

%By iterating over the queue, developers can easily write simple adaptation strategies such as dropping messages larger than size $S$, every $N$ messages, or first $N$ messages. Alternatively, they can change the order of messages, e.g., moving the high priority message from end to front of the queue. Moreover, since \system supports a flexible scripting language interface, they can also develop more complex logics. For example, one can transform payload of messages with external services, using features that are not built-in such as compressing video frames. 


%The same interfaces of adapting prior request can be used for adapting new requests. Similarly, developers can set triggers on their desired metrics and modify the new request with similar operations, as shown in Figure \ref{lst:sample} Lines \shadi{XXX}.






==> text/eval-fugu.tex <==
\subsection{Case study: video streaming}
\label{sec:eval_fugu}

% (1) what does the application do, and how is it structured?
For our second case study, we run the Fugu~\cite{yan-nsdi20} video-streaming server, which has been developed as part of the Puffer project\footnote{\url{https://puffer.stanford.edu}}. As with common streaming protocols like HLS and MPEG-DASH, Fugu divides a source video into self-contained, fixed-length segments or chunks, and transcodes each chunk into five to ten resolutions. Servers typically break up streams into four- to ten-second chunks and encode with H.264 or H.265.  

Unlike traditional approaches to adaptive-bitrate streaming (ABR), Fugu places its adaptive intelligence at the server instead of the client. Fugu clients poll the server for chunks without specifying a resolution, and Fugu responds to a poll when a client's playback buffer falls below 15 seconds. The Fugu server sends chunks at the highest resolution it predicts will arrive in time for playback. These predictions are based on the previous five chunks' transmission times and low-level TCP information. Fugu feeds these inputs to a deep neural network (DNN) trained on months of user traces, and the DNN outputs a distribution of transmission times for each chunk resolution. 
%These distributions contain probabilities for transmission time range in 500\unit{ms} granularity. 

% (2) what problems does network variability and disconnection cause for the (unmodified) application?
% Fugu performs well *mostly* 
Fugu outperforms prior approaches to ABR because it explicitly considers transmission time. In contrast, Pensieve~\cite{mao-sigcomm17} and other ABR systems estimate bandwidth using transmission sizes. And yet even though Fugu is best-in-class, it struggles when bandwidth is low. The worst outcome for a video server is client stalling~\cite{dobrian-sigcom11}, and over an eight-month period the Fugu operators observed that 83\% of stalls occurred when the average throughput was less than 6\unit{Mbps}~\cite{yan-nsdi20}. Furthermore, streaming over a low-bandwidth connection was not uncommon, accounting for 14\% of overall viewing time. 

\begin{figure}[t]
  \begin{lstlisting}[style=lua,xleftmargin=13pt]
  function envoy_on_response(h)
    -- estimated BW by BumbleBee
    bw = queue:getBW()
    for item in queue:getItem() do
      age   = item:getAge()
      size  = item:size()
      resol = item:getHeader("resolution")
      ptt   = item:getHeader("ptt")
      dur   = item:getHeader("duration")
      -- estimated transmission time (ett)
      ett   = size / bw
      -- decision mechanism
      if ett > ptt || age > dur then
        -- select appropriate resolution to
        -- downsample
        new_res, new_ett = 
          computeEttPred(resol, ptt, ett, age)
        if new_res ~= resol then 
            item:transform(new_res)
        end end end end
  \end{lstlisting}
  \caption{This \system script for Fugu downsamples video chunks if the estimated transmission time (ett) is greater than the predicted transmission time (ptt) or if the chunk duration is greater than the time it has already spent in the queue.}
  \label{lst:Fugu}
  \end{figure}


%Such streams accounted for 14\% of overall viewing time and 83% of stalls.
%at the tail of stall time distribution, more than 0.8\% streams stall when estimated throughput is  

%This represents approximately 30 seconds stall in an hour long
%video streaming. However, in supporting a large number of users, the streaming
%service experiences outrage almost 3 days per year, which is unacceptable
%stall, outrage duration to commercial services. % 0.008*365=2.92 days

%When a server sends low-resolution chunks, bandwidth estimates will not accurately capture the potential improvement of current bandwidth. Using raw network statistics from TCP sockets, and combined with history of past recent transmission, Fugu makes a good prediction and outperforms prior systems in resolution of video and the total stall times, i.e., the duration of video playback is frozen due to empty playback buffer.

% problem: head-of-line blocking when BW drops
\begin{figure*}[t]\centering
  \begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\columnwidth]{figs/bw-smoothed-s0.pdf}
  \caption{S0 Bandwidth Estimation}
  \label{fig:fugu_s0_ts_bw}
  \end{subfigure}
  \begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\columnwidth]{figs/s0_buf.pdf}
  \caption{S0 Playback Buffer}
  \label{fig:fugu_s0_ts_buf}
  \end{subfigure}
  \begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\columnwidth]{figs/cdf_s0_res.pdf}
  \caption{S0 Video Resolutions}
  \label{fig:fugu_s0_cdf_res}
  \end{subfigure}
  % \caption{Short trace 0 (S0)}
  % \label{fig:fugu_s0}
  % \end{figure*}
  % \begin{figure*}[t]\centering
  \begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\columnwidth]{figs/bw-smoothed-t10.pdf}
  \caption{L0 Bandwidth Estimation}
  \label{fig:fugu_t10_ts_bw}
  \end{subfigure}
  \begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\columnwidth]{figs/t10_buf.pdf}
  \caption{L0 Playback Buffer}
  \label{fig:fugu_t10_ts_buf}
  \end{subfigure}
  \begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\columnwidth]{figs/cdf_t10_res.pdf}
  \caption{L0 Video Resolutions}
  \label{fig:fugu_t10_cdf_res}
  \end{subfigure}
  \caption{\system helps Fugu adapt under a short trace (S0) and a long trace (L0).
    Figures in the first column show the bandwidth estimates for both traces. Figures in the second column show how the client's playback buffer changes during the trace. For both Fugu (FG) and Fugu with \system (BB) traces, \system helps Fugu eliminate stalling. Figures in the third colum show CDFs of video resolution. Under \system, Fugu sacrifices some video resolution to eliminate stalling. 
  }
  \label{fig:fugu_t10}
  \end{figure*}

Head-of-line blocking is the primary culprit for stalled playback. When bandwidth suddenly drops, higher-resolution chunks that Fugu starts to transmit under good network conditions clog the connection and block chunks behind them. This phenomenon happens for two reasons. First, Fugu updates its network estimates when transmissions complete. Thus, when bandwidth suddenly drops in the middle of a slow transmission (e.g., sending a high-resolution chunk under limited bandwidth), Fugu will continue to send the client high-resolution chunks until a slow transmission completes. The worse the misprediction, the longer it takes Fugu to correct its bandwidth estimate, and the more mispredicted chunks Fugu will try to send. Second, even after a slow transmission completes and Fugu recognizes that conditions have suddenly changed, it has no way to correct its mistakes. Fugu cannot alter or cancel the high-resolution transmissions it sent using incorrect bandwidth estimates. 

Fortunately, the concise \system script in Figure~\ref{lst:Fugu} allows Fugu to monitor enqueued chunks' ages and adapt to sudden bandwidth changes by downsampling chunks when delays rise above a threshold. The Fugu script differs from the traffic-monitoring script in Figure~\ref{lst:yolo} in two noteworthy ways. First, Fugu iterates over enqueued responses rather than requests. Second, Fugu must provide additional context to its Lua script through HTTP-header fields, including a chunk's resolution, its duration, and its predicted transmission time. Figure~\ref{lst:yolo} and Figure~\ref{lst:Fugu} are otherwise similarly concise and readable.

% (3) what BumbleBee code did we write to help it deal with the problems described above?



%As before, the Fugu script iterates over enqueud When age of a chunk is above pre-defined threshold and/or estimated current
%bandwidth is insufficient to transmit within the chunk's predicted time, it
%downsamples a chunk via {\tt transform()} function. In current version, we
%choose to use 4s as a threshold by default, as each chunk is 4s long.
%Transforming a chunk into lower resolution reduces the size of data to
%transmit, even if bandwidth sharply drops, or Fugu makes a wrong prediction.
%Therefore, \system alleviates the head-of-line blocking problem by massaging
%the data, adapting to current network conditions.


% (4) Describe the experiments we ran to validate whether BubmbleBee helped
% mitigate those problems? 
To evaluate \system-enabled Fugu under representative network conditions, we analyze Puffer traces from January 2020, focusing on the nine sessions that exhibit the most client stalling. Using these session logs, we estimate instantaneous bandwidth to emulate network conditions for a client watching a video. We smooth bandwidth estimation over ten second windows, which is the finest-grained control supported by our network-emulation tool. Among the nine session traces from Puffer, six last less than 10 minutes, two are approximately 20 minutes long, and one is an hour long. We use the traffic video from Section~\ref{sec:eval_yolo} as a source video and divide it into four-second chunks.

% (5) Describe the results of the experiments we ran. For each graph, describe
%     the x and y axes, describe what each bar/line/boxplot represents, describe
%     the most important take-away and why it makes sense, and explain any
%     surprising/counter-intuitive results and why they make sense.

We first characterize Fugu's behavior under a short trace (S0) and a one-hour trace (L0).
Figure~\ref{fig:fugu_s0_ts_bw} shows the raw and smoothed bandwidth for S0, and
Figure~\ref{fig:fugu_t10_ts_bw} shows the same for L0. The graphs show that bandwidth varies by half an order of magnitude in S0, and by a full order of magnitude for L0. 

%The results explain the tail of stall time distribution for Fugu from making prediction with the past good network conditions, and tolerating the head-of-line blocking problem. On the other hand, the results suggest a potential improvement that \system can achieve by mitigating HOL blocking problem.

Next, we characterize Fugu with and without \system using two metrics: playback buffer and video resolution. The playback buffer represents seconds of video that a client can play without receiving new data from the server. When the buffer reaches zero, the video stalls. Resolution represents video quality. Buffer and resolution can be traded off. In the extreme, sending only low-resolution chunks minimizes quality but maximizes buffer, whereas sending only high-resolution chunks maximizes quality but minimizes buffer. Because stalls are so painful~\cite{dobrian-sigcom11}, \system wants to offer acceptable quality and no stalls.

Figure~\ref{fig:fugu_s0_ts_buf} shows that even though S0 has less bandwidth variability than L0, Fugu's playback buffer often drops to zero. In comparison, \system's playback buffer never drops to zero and maintains between 10 and 20 seconds of buffer throughout the trace. Eliminating stalls requires lower-resolution video, and Figure~\ref{fig:fugu_s0_cdf_res} shows a CDF of video resolutions for Fugu with and without \system. \system allows Fugu to utilize a wider range of resolutions, but at the 75th percentile, Fugu without \system delivers twice the resolution. We believe that this is an acceptable trade-off for eliminating stalls.

\begin{figure}[t] \centering
  \begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\columnwidth]{figs/boxplot-buffer-pf-bb.pdf}
  \caption{Across all traces, playback buffer levels are more consistent with \system than without. \system also allows Fugu to eliminate all stalls (no buffer sizes of 0 with \system).}
  \label{fig:fugu_bar_buffer}
  \end{subfigure}
  \begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\columnwidth]{figs/boxplot-resolution-pf-bb.pdf}
  \caption{To eliminate stalls, \system sacrifices some video resolution.}
  \label{fig:fugu_bar_resolution}
  \end{subfigure}
  \caption{Experiments with the nine Puffer traces with the most stalls from January, 2020 (six short and three long) show how \system helps Fugu eliminate stalls while maintaining acceptable video resolution.}
  \label{fig:fugu_bar}
  \end{figure}
Figure~\ref{fig:fugu_t10_ts_buf} shows that \system also eliminates stalling under the longer L0 trace. \system allows the client to maintain a playback buffer of close to 15 seconds for the duration of L0. Interestingly, Figure~\ref{fig:fugu_t10_cdf_res} shows that for L0 the 60th percentile resolution for Fugu with and without \system are equivalent. This is because \system only acts when Fugu mispredicts a chunk's transmission time. When bandwidth is good enough to transmit within a chunk's deadline, Fugu's decisions are correct and \system does nothing. In other words, \system does not adapt 40\% of the time.

Figure~\ref{fig:fugu_t10_ts_buf} is most interesting between 1700s and 2100s. Around 1700s, bandwidth drops from 100\unit{KBps} to 20\unit{KBps}. \system adapts and the playback buffer remains consistent. However, without \system Fugu is in the middle of transmitting a high-resolution chunk when the bandwidth drops. Fugu continues sending high-resolution chunks until a slow transmission completes and it updates its bandwidth estimate. However, while Fugu works through its backlog of high-resolution chunks, it begins to send low-resolution chunks based on the updated transmission times. These smaller chunks compete for limited bandwidth with the remaining larger chunks. The smaller chunks stall for so long that Fugu sends over twenty more to catch up. However, at time 2100s, bandwidth suddenly recovers and the backlog of low-resolution chunk transmissions quickly complete, causing the client's buffer to swell to nearly 90s. This period in the experiment demonstrates how failing to adapt to sudden bandwidth increases wastes resources. A better strategy would have been to use the additional bandwidth to deliver higher-resolution chunks instead of creating a nearly 90s playback buffer. \system fully utilizes the available bandwidth by upsampling videos to match the most recent network observations.

%% main takeaway: BB has less variances.
Figure~\ref{fig:fugu_bar_buffer} summarizes playback buffer levels for all nine traces. Each boxplot represents 25th and 75th percentiles with black median bar and min and max wisps. The results show that \system has less buffer variance and no stalls across every trace. Figure~\ref{fig:fugu_bar_resolution} summarizes resolution for all nine traces.
Each boxplot represents 25th and 75th percentiles with black median bar and min and max wisps. These results show that \system allows Fugu to use a wider range of resolutions. 
For example, for the M1 trace, \system utilizes four different resolutions between 144p and 2160p. On the other hand, without \system Fugu uses the highest resolution throughout entire M1 trace. For the shorter traces (i.e., S0-S6), Fugu has so many stalls that the box charts span a wider range. However, as shown in Figure~\ref{fig:fugu_s0_cdf_res}, \system switches between more resolutions than Fugu.

%Fugu without \system switches resolutions more than with \system. This is because Fugu's prediction attempts to spot an
%instantaneous throughput and selects suitable resolutions to transmit over a
%short time horizon. \shadi{Agree that this exaplanation doesn't make sense.}

\begin{figure}[t]
  \includegraphics[width=\linewidth]{figs/stallratio-vs-avgres.pdf}
\caption{\system allows Fugu to eliminate stalling with acceptable drops in mean video resolution. Each color represents a trace, with the circle showing results for Fugu without \system (FG) and the star showing results for Fugu with \system (BB). When mean resolution for Fugu is below 1080p, adding \system eliminates stalling with negligible drops in mean resolution. For traces with higher mean resolution, \system reduces mean resolution by at most 24\% for S3.}
\label{fig:fugu_stallvsres}
\end{figure}

Figure~\ref{fig:fugu_stallvsres} provides an overview of how \system helps Fugu eliminate stalls. The X-axis is the ratio of total stall time, i.e., the percent of time a video stalled. The Y-axis is mean resolutions in pixels. Each color represents a trace, with the circle showing results for Fugu without \system (FG) and the star showing results for Fugu with \system (BB). When mean resolution for Fugu is below 1080p, adding \system eliminates stalls without affecting resolution. For traces with higher mean resolution, \system must sacrifice more resolution to eliminate stalling. In the worst case of S3, \system reduces mean resolution by 24\%. In the best case, S5, \system reduces mean resolution by only 6\%. In comparison, Fugu without \system results in 5\% stall time in the best case and 83\% in the worst case.

To summarize, \system allows Fugu to eliminate stalling while maintaining acceptable video resolution. We also show that the adaptation strategies responsible for these benefits can be concisely expressed by the script in Figure~\ref{lst:Fugu}. Finally, it is important to note that we added \system's adaptive logic to Fugu without modifying its code. Inter-operating with unmodified code is especially valuable for containerized applications and orchestration platforms.

%Interestingly, for S0 and T0, \system reduces stall ratio with no decrease in mean resolution. We suspect two reasons. First, in S0 case, Fugu transmits high resolutions when possible while \system fluctuates in a combination of resolutions. Secondly, in T0 case, Fugu and \system's tail resolutions converge; when Fugu experiences stall time, \system transmits significantly lower resolutions.

% Thus, \system embraces high variability of available bandwidth by trading resolutions for better playback buffer level.

% \input{text/eval-iot.tex}

% (1) what does the application do, and how is it structured?

% (2) what problems does network variability and disconnection cause for the (unmodified) application?

% (3) what BumbleBee code did we write to help it deal with the problems described above?

% (4) Describe the experiments we ran to validate whether BubmbleBee helped mitigate those problems? 

% (5) Describe the results of the experiments we ran. For each graph, describe the x and y axes, describe what each bar/line/boxplot represents, describe the most important take-away and why it makes sense, and explain any surprising/counter-intuitive results and why they make sense.





==> text/eval-iot.tex <==
\subsection{Engine diagnostics}
\label{sec:eval_engine}

Our last set of experiments is with a predictive maintenance application~\cite{predictive-maintenance}. The application feeds sensor data from an aircraft with two simulated engines to an ML model that predicts an engine's remaining useful lifetime (RUL). Each engine streams data from 26 sensors to the cloud. The cloud archives the sensor data to retrain the ML model, displays the data on an operator dashboard, and forwards the data to the ML model to predict its RUL. If either the operator or ML model detects something predictive of near-term engine failure, the plane should land as soon as possible. 

Flights typically last between two and ten hours, and an aircraft should update its RUL every 30 minutes. According to XXX aircraft engines generate XXX Mbps of sensor data that should be transmitted to the cloud. 

The application running at the cloud takes input streams from
sensors in turbofans, and monitors the engines' remaining useful life (RUL).
When RUL falls below a threshold indicating a potential likelihood of
failures in the future, the application notifies and recommends the field
engine mechanics for an immediate inspection. Note that the application is out
of the mission-critical operations, for which running locally with low
fidelity like the traffic monitoring application does is better and more
reliable.

Unfortunately, the network environment that sensor streams are generated and
uploaded from experience frequent disconnetion~\cite{noghabi-getmobile20}.
% Unlike handheld mobile devices that are highly and reliably connected to
% today's cellular networks
Even for a short period of connectivity, the application may result in a long
service interruption when network is reconnected. 
This is because that sensors continue to generate streams even during
disconnected from networks, and those old streams are waiting in the queue to
flush. In other words, when disconnected for a period of time, the bulk of
stale, old streams is buffered in the queue. So, when reconnected, the bulk of
stale streams at front of the queue is transmitted first.  Consequently, new
sensor streams experience a high queueing delay.

Dropping old streams is one solution to reduce the queuing delay; the field
mechanics may require old archival data to prune, or simply to collect for
analytics purpose. Another approach is sending new streams first with
available bandwidth, and utilize surplus bandwidth to periodically upload old
streams in background. This approach requires the application to monitor the
network conditions and act accordingly~\cite{aruna-sigcomm07,
higgins-mobicom10}.

Recall that the stream application has no control over the orders of queued
streams. That means, even with a precise network monitoring, the application
may still experience a high latency. For example, when network disconnects in
the middle of uploading new streams, the application has no method to cancel
currently buffered streams in the queue. As a result, new streams in the queue
impose queueing delay for uploading later streams when network recovers later.

\begin{figure}[t]
\begin{lstlisting}[style=lua,xleftmargin=13pt]
function envoy_on_request(h)
  -- if queuing delay exists
  if queue:length() > 1 then
    h:pushFront()
  else
    h:pushBack()
  end
end
\end{lstlisting}
\caption{This simple Lua script for the sensor stream application alternates
between FIFO (First In, First Out) and LIFO (Last In, First Out).}
\label{lst:iot}
\end{figure}

\system assists the application by empowering an ability to alter the orders
within the queue. Specifically, the application developers configure the queue
to switch between FIFO and LIFO, depends on the length of the queue as little
as 4 LoC shown in Figure~\ref{lst:iot}. We evaluate the efficacy of \system's
simple reodering by measuring run-time, i.e., time delta between when data
were generated and when successfully uploaded to the cloud.  We simulate
real-time sensor streams by replaying NASA PCoE
Dataset~\cite{turbofan-dataset}. The dataset contains 100 sensors generating
streams at 10\unit{ms} interval. We configure the sensors to scale-up to 6x to
reflect realistic workloads. We also instrument sensors to report streams to a
central router that periodically uploads aggregated sensor streams at
2\unit{s} interval to Azure Blob storage.  The median and mean sizes of
aggregation are 466\unit{KB} and 487\unit{KB}, respectively. We replay the
application twice with and without \system for 20 minutes. When connectivity
is available, we limit bandwidth to 6\unit{Mbps}, according to reported uplink
conditions in US cellular networks environment~\cite{noghabi-getmobile20}. \shadi{is it cellular or satellite?}

\begin{figure}[t!] \centering
\includegraphics[width=\columnwidth]{figs/iot-ts.pdf}
\caption{The comparison of run-time for uploaded sensor streams.  w/ BB refers
to \system that reorders messages in the queue. w/o BB refers to the baseline
application. }
\label{fig:iot_ts}
\end{figure}

Figure~\ref{fig:iot_ts} is the result of experiment. The X-axis is an epoch
when a stream is generated. The Y-axis is run-time of streams in log scale. We
set the disconnection for 5 minutes between 300 and 600 epochs. The result
suggests that \system's reordering adaptation alleviates the queueing delay
imposed by old streams waiting in the queue. For example, when connectivity
recover at epoch 600s, \system stabilizes run-time to previous level
immediately whereas the baseline application suffers from high queuing delay
until 750s. Interestingly, the run-time of streams generated during
disconnection converges at 500s. This is because with \system, the application
efficiently utilizes surplus bandwidth left after priortizing new streams over
old streams. From the log, we confirm that with \system, the queue becomes
empty 89s later than without \system.

To sum up, our last set of experiments with predictive machinary diagnostics
application indicates that the efficacy of \system's very simple reordering
adaptation technique is beneficial.  In particular, applications sensitive to
queuing delay in respect to network connecitivty can significantly benefit
without losing old streams for archival and pruning purposes.



==> text/implementation.tex <==
\section{Implementation}
\label{sec:impl}
%In this section, we describe the implementation in details to apply
%aforementioned design principles in a service-mesh architecture. We start with
%a high-level overview of a sidecar proxy, Envoy that our prototype system is
%built upon. Next, we discuss \system's basic architecture to support an array
%of adaptation strategies enabled by the generic queue abstraction. Then, we
%cover how to add the adaptation programmability in \system. We conclude the
%section with putting implementations altogether.



%\subsection{Sidecar Proxy}

\label{sec:envoy}

\begin{figure}[]
	\centering
	\includegraphics[width=\columnwidth]{figs/envoy.pdf}
	\caption{Envoy's Architecture in a single pod.}
	\label{fig:envoy}
\end{figure}

\begin{figure}[]
	\centering
	\includegraphics[width=0.9\columnwidth]{figs/envoy-BB.pdf}
	\caption{{\name}'s integration with Envoy}
	\label{fig:envoy-with-BB}
\end{figure}


%This section describes the implementation details of {\name}.

{\name} is implemented as an addition to of Envoy~\cite{envoy}, a sidecar proxy in container-orchestration platforms, such as Borg~\cite{verma-eurosys15} and Kubernetes~\cite{hightower-oreilly17}.
As shown in Figure \ref{fig:envoy}, in every application pod, an Envoy container is placed alongside other application containers. Envoy intercepts all network packets to/from the application containers by injecting {\tt iptable} rules at a startup time.
Inside Envoy, these redirected messages go through a chain of pre-configured \emph{filters}. Filters have full control over messages and can perform various operations on them, such as redirecting to another destination, dropping messages, or transforming the payload. 

Envoy works fully transparently, without the need for any application modification (unlike many prior systems~\cite{noble-sosp97, fox-asplos96}), making it an ideal location to add {\name}'s adaptation. We implemented {\name} in Envoy by adding two components, a {\name} filter and queue manager, as shown in Figure \ref{fig:envoy-with-BB}. \shadi{add the flow for callbacks in Figure \ref{fig:envoy-with-BB}}.
We have implemented \system on top of Envoy v1.12 with $\approx$ 2900 lines of code (LOC).
We have modified Envoy for only 103 LOC to add features such as modifying headers by function pointer. 


\noindent \textbf{{\name} queue manager:} 
%\subsection{{\name} queue manager}
Envoy acts as a stateless layer -- it creates a filter thread per message which is destroyed after the message is dispatched. On the contrary, {\name} exposes a persistent and modifiable message queue abstraction, which requires state across messages. Therefore, {\name} includes a separate global thread, the queue manager, that persists throughout the lifetime of the Envoy container. After messages go through {\name}'s filter, they are enqueued the queue manager until they are ready to be delivered. 
The queue manager dequeues messages and transfers them back to {\name}'s filter, which then the messages traverse the remaining filters registered in Envoy. The queue manager maintains a queue per destination pod plus an additional default queue for undefined destinations, e.g., outside the local cluster.

The queue manager also enforces a rate-limit per destination using a token-based approach to avoid bandwidth saturation by malicious applications. We currently support rate limiting in \unit{KB/s} granularity.


%\shadi{is there Queue per connection? envoy container?} 
%\joseph{Queue per destination. We have default queue + N queues pre-defined destinations. You can think as queue per destination pod.}
%\shadi{"to ensure repeatable
%simulation in network conditions changing when configured over an order of
%seconds window", @Joseph: huh?}
%\joseph{rate-limit can be changed every a few seconds, unlike Linux TC that can change every milliseconds.}

\noindent\textbf{\system filter:} 
The \system filter enables developers to a) apply their custom adaptation logic on on-the-fly messages (enqueued in the queue manager) or new messages and b) to register callbacks on user-defined triggers. 
% Envoy intercepts the level L3 (TCP) to L7 (HTTP) network messages,
% however, our current implementation of \system is operating at the HTTP level.
% At this level, the boundaries of requests and responses are well-defined. With
% minimal additional burden on the developers (to define boundaries), \system
% can easily be extended to operate at lower levels.
%\joseph{
%Envoy intercepts all communication messages
%in a service-mesh topology. 
%Our current prototype of \system operates at the
%HTTP layer, even though fundamentally, \system works at much lower layers such
%as TCP. We have implemented at the layer, because it offers a clear
%boundary per message, and this significantly reduces our engineering effort.}
%
Our current implementation of \system operates at the HTTP layer since this layer provides a clear boundary per message. However, envoy intercepts all communication messages and with additional engineering effort \system can easily be extended to lower layers (e.g., TCP).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textit{Queue and message adaptation:} \system supports
a wide and flexible range of adaptation strategies. Developers can write any custom Lua script adaptation logic (Section
\ref{sec:design}) to transform i) the content of each message (header and payload),
and ii) the structure/order of the queue of messages. Application developers register entry points via {\tt envoy\_on\_\{request/response\}} hooks
for egress/ingress messages.
\system automatically
executes the user's Lua script on the enqueued data. To prevent race
conditions, in each queue of messages, a small portion at the head and tail
are marked as immutable (shown in red in Figure \ref{fig:envoy-with-BB}). The
adaptation is only applied to the mutable portion of the queue (shown in green
in Figure \ref{fig:envoy-with-BB}).

To achieve fast adaptation, \system  performs transformations in an asynchronous manner. The adaptation script proceeds with following messages in the queue after invoking the {\tt transform()} function (in a non-blocking manner). Later on, the outcome of transformation replaces the payload of messages while preserving the order of items in the queue.
 
 
Internally, the \system filter leverages Envoy's built-in message interfaces,
such as  {\tt encodeHeaders()} and {\tt decodeData()}, to intercept ingress
and egress message headers and payloads. For example, \system enables
rerouting messages to an alternative destination. This is done by modifying
the {\tt :HOST} field in the header. Note that at the HTTP layer, the header
is stateless (as opposed to connection-based protocols like TCP) and can
easily be configured to an alternative destination. 

%In addition, \system exposes additional functionality to modify the structure
%or order of the queue, e.g., moving data from the front of the queue to the
%back. The currently supported functions are \shadi{... what are the APIs
%allowed?} \shadi{maybe move this to programmability section?}
%
%\shadi{ I am not sure that i fully understood what message you planned to
%convey in the following points. I rewrote what I understood.} 
%\joseph{The purpose of above paragraphs is to deliver a background on how
%Envoy's HTTP filter works. The last paragraph works like a bridge, giving a
%clue about simple in-network operations like dropping, reordering. Up to this
%point, there's no discussion about callbacks, transformation, and
%programmability.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textit{Callbacks:} Application developers
can register callbacks to set of endpoints on changes in network conditions, e.g., to adjust a
sensor's reporting interval when network conditions are poor. \system uses REST end-points for callbacks. When the conditions of a callback are met, the \system filter automatically posts the callback on the registered REST endpoint(s) along with the registered metrics.

% \system allows registering callbacks on network metrics, notification
% conditions, and REST end-points at the startup time 
% \shadi{@joseph, what is notification conditions and rest endpoints?}. 
% \joseph{Two ways to get notified. (1) specify in if-else statement
% e.g., notify /XXX if bw < 25Mbps, or (2) use BB's notify function as shown in
% Figure 3 line 23.  Currently, we support only BW changes.  REST endpoints are
% really app-dependent (e.g., in python-flask, 
% {\tt @app.route('/notify', methods=['POST', 'GET'])})} \shadi{not sure what is the diff between 1 and 2?}

%To use callbacks, application developers need to define a callback reference that
%contains a) the list of endpoints to trigger a callback on, and b) the list of
%metrics to capture and include in the callback.  This callback reference is registered by defining the trigger condition and calling the {\tt notify()} function in the Lua script. 
%Figure \shadi{XX} shows an example of a \shadi{XX} application using callbacks to \shadi{XX}.
%

%\system filter continuously monitors triggers defined for callbacks. When
%the conditions of callbacks are met, the filter automatically notifies the
%application over asynchronous REST APIs. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\noindent \textbf{Exposing low-level networking metrics:} A main advantage
%of running adaptation in-network is the enhanced visibility an application
%can have on low-level networking metrics, e.g., queue size. \system exposes a
%comprehensive set of such metrics (Section XX). In addition, since latency is
%one of the main metrics for adaptation, \system exposes two additional latency
%metrics: i) end-to-end latency, as time difference between the request being
%received and corresponding response being sent at Envoy and ii) message age,
%as the time spent in \system's Queue. 
%These latency metrics are added to the header field of messages as {\tt
%bb-e2e-latency} and {\tt bb-age}. 
%\shadi{1.are these the only latency metrics available to the users? 2. why is
%it important that we are exposing these latency metrics, e.g., why isn't the
%queue size equally important } 
%\joseph{1. we also expose TCP metrics (we had to for Puffer). Let me know if I
%  missed other metrics. 
%  2. queue size can be equally important to some applications. What I was
%  trying to highlight was that because BB is operating at in-network level,
%  latency can be broken down in fine granularity. }
%\shadi{I feel this this is not including all that should be included. are
%there other things missing? }
%\joseph{Let me think about other missing metrics.}



%\squishlist
%	\item \textit{rerouting of messages to an alternative destination:} 
%	when the original destination becomes overloaded or disconnected.
%	This is done by modifying the {\tt :HOST} field in the header. At the HTTP layer, the header is stateless (as opposed to connection-based protocols like TCP) and can easily be configured to an alternative destination.
%	\item \textit{exposing latency in the messages:} since latency is one of the main metrics for adaptation, \system two latency metrics: i) end-to-end latency, as time difference between the request being received
%	and corresponding response being sent at Envoy and ii) message age, as the time spent in \system's Queue. 
%	\system exposes the latency metrics in the header field as {\tt bb-e2e-latency} and {\tt bb-age}. These latency metrics, alongside other low-level networking metrics such as queue size, can be used by developers to define custom adaptation strategies using \system's scripting interface (Section ??).
%	 \shadi{@joseph, these metrics are not clear. I tried to write them precisely but I am not sure they are correct. Can you check and fix?} \shadi{1.are these the only latency metrics available to the users? 2. why is it important that we are exposing these latency metrics, e.g., why isn't the queue size equally important }
%	\shadi{I fell this item does not belong here. @Joseph: is there a reason you included this here?}
%	\item \textit{callbacks to applications:} Application developers can register callbacks on changes in network conditions, e.g., to adjust a sensor's reporting interval when network conditions are poor. \system allows registering callbacks on network metrics, notification conditions, and REST end-points at the startup time \shadi{@joseph, what is notification conditions and rest endpoints?}.
%	Listing \shadi{XX (@Joseph: please add)} shows an example of such callbacks. The \system filter notifies the application over asynchronous REST APIs when the conditions of the callbacks are met. 
%	
%\shadi{I feel this this is not including all that should be included. are there other things missing? }
%\squishend


%%%%%%%%%%%comments%%%%%%%%%%%%%%%





% \shadi{@Joseph: in figure 1, instead of filter 1...3, maybe, we can have actual filters used in current setup? Like Router filter, Logging filter, etc, citing the list of HTTP filters \url{https://www.envoyproxy.io/docs/envoy/latest/api-v2/config/filter/http/http}}
% \joseph{JOSEPH-TODO}


%\joseph{a few minor things: 
%1) envoy intercepts the level L3 (TCP) to L7 (HTTP) network messages and our current setup intercepts only L7 messages. 
%2) usually, a Pod contains 1 application container AND 1 envoy container. So figure 1 should be N pods containing 1 app container and 1 envoy. In envoy, each queue thread is for destination. You can think destination as another pod to communicate (e.g., cloud object detector vs edge object detector). 
%3) in figure 1, instead of filter 1...3, maybe, we can have actual filters used in current setup? Like Router filter, Logging filter, etc, citing the list of HTTP filters \url{https://www.envoyproxy.io/docs/envoy/latest/api-v2/config/filter/http/http}. 
%}  
%\shadi{1. plesae check if the new text is fine. 2. I thought it doesn't have
%to be one container per pod? i was just showing one pod in that figure to
%avoid making it complicated 3. please change the figures accordingly. The raw
%files are in resources/excel-ppt/ folder. }
%\joseph{1. except for callbacks, the text is fine.
%2. You're correct and we don't have to complicate the figure. It's just a
%convention to have one app container per pod. 
%3. I'll do :-> (I even didn't know git accepts .pptx files)}


%Envoy~\cite{envoy} is a sidecar proxy in container-orchestration platforms
%like Borg~\cite{verma-eurosys15} and Kubernetes~\cite{hightower-oreilly17}.
%Envoy container is co-located with an application container, and it
%intercepts network packets to/from the application container by injecting
%{\tt iptable} rules at a startup time. In Envoy, the redirected messages go
%through a chain of pre-configured \emph{filters}. Each filter performs
%diligent operations on messages such as redirecting to another destination,
%dropping stale messages, or transforming payload of incoming messages. This is
%possible as a filter has full control over passed messages, including header
%and payload. Additionally, Envoy requires no application modification to work
%with, unlike prior systems~\cite{noble-sosp97, fox-asplos96} that require
%significant changes in applications' source code to relay messages through a
%local proxy.
%
%At the first glance, Envoy filter is an ideal place to implement the
%adaptation layer; we find that Envoy filter is stateless by its design choice.
%As a result, Envoy creates a filter thread per message, and destroys the
%thread when the message is dispatched, unlike a global TCP state shared with
%multiplexed connections (e.g., HTTP/2, WebSocket) over a full duty cycle. The
%stateless design imposes a challenge to expose a persistent message queue
%abstraction to the adaptation layer. 

%Fortunately, Envoy container survives throughout a lifespan of the application
%container, and thus, is stateful. We have implemented global queue manger
%thread in Envoy that persists throughout the duty cycle. The manager thread
%appends new messages to its queue before a filter thread is discarded by
%Envoy. Also, the manager thread enforces rate-limit per destination to avoid
%bandwidth saturation by malicious applications, and to ensure repeatable
%simulation in network conditions changing when configured over an order of
%seconds window.  The manager thread limits the bandwidth by periodically
%checking the token-bucket. Once it obtains enough tokens to transmit the first
%item in the queue, the manager thread invokes Envoy's event dispatcher to
%transmit the message. Our current implementation enforces bandwidth limit in
%\unit{KB/s} granularity, and checks the token bucket at 1\unit{ms} interval.

%\subsection{\system Filter in Envoy}
%\label{sec:filter}
%In this subsection, we describe \system filter that supports various
%adaptation strategies. 
%\system filter registers callbacks to intercept the
%level-seven message header and payload for ingress and egress messages via
%Envoy's well-defined interfaces such as {\tt encodeHeaders()} and 
%{\tt decodeData()}.

%Rerouting to alternative service is a form of adaptation strategies enabled by
%\system. For example, when service A is over-loaded, rerouting to service B
%or to local service can be desirable for low latency. To achieve the rerouting
%feature, we leverage the header field in the level-seven message structure.
%As opposed to connection-oriented protocols like TCP, the level-seven message
%is stateless and can be configured easily to send alternative sinks. \system
%filter modifies {\tt :HOST} field in the header so that when Envoy's event
%dispatcher reads a destination to transmit, the modified host destination is
%selected. 

%In many cases, the end-to-end latency is one of main performance metrics that
%applications care about. For instance, object detection application may have a
%service-level agreement for its tail latency. If a model's detection latency
%approaches the tail, it can use a cheaper model to trade accuracy for latency.
%\system filter exposes two types of latency: the end-to-end latency, and
%fine-grained network latency such as queuing delay, transmission delay, etc.
%The former can be measured by the application itself; the later is only
%possible by in-network system like \system. We record timestamps for request
%message coming in and corresponding response message transmitted. We define
%{\it age} of a message for how long it has been in the queue whereas we
%compute the end-to-end latency for a delta between ingress message received
%and egress message sent. \system exposes these latency metrics in the
%level-seven's header field {\tt bb-e2e-latency} and {\tt bb-age}.

%Application-collaborative adaptation~\cite{noble-sosp97} allows the underlying
%system to notify the application about changes in execution environment, and
%let it adapt internally. For example, sensor monitor application running on
%inexpensive IoT device has limited local storage that buffers data that could
%have not been sent instantaneously.  When uplink network is saturated, the
%application can adjust a frequency of sensor data collection to avoid running
%out of local storage if notified about the network changes.  Application
%developers can register network metrics, notification conditions, and REST
%end-points at the startup time. \system filter notifies the application over
%asynchronous REST interfaces when the conditions for pointed metrics are
%satisfied. Note that even without application collaboration, \system filter
%still works; the collaboration allows applications to adapt internally with
%better knowledge about data and their objectives.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Programmability in \system}
%\label{sec:lua}
%
%%\system exposes an imperative adaptation interfaces in Lua scripting language.  The use of imperative interfaces removes the need of
%%platform-dependent implementations and interrupting services when
%%rolling out new strategies. Moreover, application developers can easily integrate their custom logics without the constrains of declarative languages, e.g., SQL.
%%
%%Application developers register entry points via {\tt envoy\_on\_\{request/response\}} hooks
%%for egress/ingress messages. The registered functions are executed per
%%message. \system provides access to both each individual messages content and headers (e.g., destination, payload size), and the global queue of messages (one queue per destination). The full list of APIs exposed by \system are shown in Table \ref{tab:bb_api}.
%%\shadi{list all the possible operations, e.g., transform (), in a table?}
%
%%By iterating over the queue, developers can easily write basic adaptation strategies such as dropping messages larger than size $S$, every $N$ messages, or first $N$ messages. Alternatively, they can change the order of items, e.g, moving the high priority message from end to front of the queue. In addition, since \system supports a flexible scripting language interface, they can also develop complex logic. For example, one can transform payload of messages with external services,
%%using features that are not built-in such as compressing video frames. 
%
%\shadi{
%Figure \ref{lst:yolo} shows an example adaptation for a video processing application which adapts to disconnections by rerouting messages (Lines 11-14) and adapts to bandwidth drops by reducing the video quality (Lines 15-18) and potentially triggering a callback to the application (Lines 20-24). More details of this scenario are explained in Section~\ref{sec:eval_yolo}.
%%
%\newline
%%
%Note that developers program their adaptation logic as if the operations were performed internally in the application and \system takes care of executing the adaptation logic whenever required.
%%
%entry points via {\tt envoy\_on\_\{request/response\}} hooks
%for egress/ingress messages.
%}
%To achieve fast adaptation, \system  performs transformations in an asynchronous manner. The adaptation script proceeds with following messages in the queue after invoking the {\tt transform()} function (in a non-blocking manner). Later on, the outcome of transformation replaces the payload of messages while preserving the order of items in the queue.



%It it important to highlight that developers program all logics as if
%performing operations internally in applications, and lowers a complexity to
%write custom strategies. We revisit a complexity of writing adaptation
%strategies in Section~\ref{sec:evaluation}.



%Empowering programmable adaptation to inter-task communication is crucial task
%to \system. As discussed in Section~\ref{sec:design_interface}, % design:Expose imperative rather than declarative adaptation interfaces 
%\system exposes imperative adaptation interfaces in Lua scripting language to
%integrate lightweight in-network processing functionality. The use of
%imperative interfaces alleviate application developers from a burden of
%platform-dependent implementation and a hassel to interrupt services when
%rolling out new strategies, like in case of updating with executable binaries.

%Application developers can easily integrate their custom logics in Lua script.
%They register entry points via {\tt envoy\_on\_\{request, response\}} hooks
%for egress and ingress messages. The registered functions are executed per
%message. When invoked, the script can not only retrieve information related to
%current message (e.g., destination, payload size), but also, can access to
%\system's global queue for the past messages in the queue. Our current
%implementation exposes a queue per route. 

%By iterating over the queue, the script performs basic operations such as
%dropping messages larger than size $S$, every $N$ messages, first $N$
%messages, and so on. In addition, it may change the order of items based on
%needs, e.g, moving the high priority message from end to front of the queue to
%allow a fast transmission.  The capability of operations reach's beyond simple
%operations. One can transform payload of messages with external services,
%using features that are not built-in such as compressing video frames. \system
%offers transformation feature via asynchronous calls. In other words, while
%the script proceeds with following coroutines after invoking {\tt
%transform()}, the outcome of transformation replaces the payload of messages,
%preserving the order of items in the queue.
%
%It it important to highlight that developers program all logics as if
%performing operations internally in applications, and lowers a complexity to
%write custom strategies. We revisit a complexity of writing adaptation
%strategies in Section~\ref{sec:evaluation}.

%\shadi{add example of Lua script adaptation}


%\subsection{Implementation of \system}
%\label{sec:impl_details}
% Envoy modification: 
%  11 files changed, 109 insertions(+), 7 deletions(-)
%  103 SLOC added
% BB filter addition:
%  12 files changed, 4340 insertions(+)
%  2876 LOC added
% TOTAL: 2979 SLOC added
%We have implemented \system filter on Envoy v1.12.0. \system filter is
%consisted of 2876 SLOC. The majority of source lines is dedicated to adding
%programmability support in \system. We also have modified Envoy for 103 SLOC to
%add features such as modifying header by function pointer. 
% testbed setup




% \shadi{@Joseph/Landon:move the following details of the setup to evaluation section:
% 	\newline"
% To apply filter configurations, we use Istio v1.4.3 on top of Kubernetes
% v1.15.10 running on Azure Kubernetes Service (AKS).
%  Our Kubernetes cluster is
% consisted of at least three nodes with 4 vCPUs 16\unit{GB} RAM, and
% 32\unit{GB} SSD. The cluster also has optional two GPU nodes with Nvidia Tesla
% K80 GPU, 6 vCPUs, 56\unit{GB} RAM, and 340\unit{GB} SSD, each.
% "
% }


==> text/intro.tex <==
\section{Introduction}
\label{sec:intro}

% compositional adaptation: orchestration
% behavioral adaptation: bumblebee
% xxx adaptation: network congestion control

The challenge of managing complex distributed applications has led to the rise of container-orchestration platforms like Borg~\cite{verma-eurosys15}, Kubernetes~\cite{hightower-oreilly17}, and Docker Swarm~\cite{swarm}. Developers configure an orchestrator with sets of physical or virtual machines, container images, and performance and reliability objectives. At runtime the orchestrator monitors application metrics and updates a mapping of named tasks to machines in order to meet the developer's objectives.

Orchestrators do their best to maintain consistent performance and reliability while keeping resource usage proportional to load. As conditions change, orchestrators can launch tasks to satisfy bursts of new requests, kill tasks when utilization drops, and load-balance traffic among tasks. However, even perfect orchestration cannot ensure good performance and reliability when machine failure, network hiccups, and under-provisioning cause resources to become scarce.

Application-oblivious responses to resource scarcity, such as TCP congestion control, try to provide fair allocation of limited resources, but only the application knows how to adjust its \emph{fidelity} under resource scarcity. For example, a machine-learning (ML) application can reduce its fidelity by switching to a simpler inference model with lower accuracy and confidence. Or a video-streaming application can reduce its fidelity by serving lower bitrate content. In each case, \emph{application-aware adaptation}~\cite{noble-sosp97} is the key to maintaining acceptable quality when resources become scarce.

%There are only three things Bumblebee can do: it can reorder application data; it can transform application data; and it can drop application data. What's (in part) interesting about Bumblebee's approach is that it can make those decisions using application semantics, using a crisp abstraction that easily fits into a containerized/service-mesh-oriented framework.

%However, the decisions Bumblebee makes are only interesting if the value of delivery is highly time-sensitive, and the time over which that value changes is short relative to the round-trip time and/or the typical disconnection time. For edge/mobile/consumer applications, those intervals are larger (because edge/consumer networks are much less reliable and performant than are institutional/infrastructure/etc.)

Unfortunately, orchestration platforms do not provide clean abstractions for application-aware adaptation. Existing network control abstractions either focus on probabilistic traffic shaping, such as load-balancing, canary testing, and A/B testing~\cite{linkerd, istio}, or are limited to stateless, per-message processing~\cite{envoy}. As a result, adaptation logic often ends up deeply integrated with the rest of an application's code~\cite{yan-nsdi20}, which makes it difficult to update or reuse adaptation strategies within container-based frameworks.

% agility and stability part isn't totally worked out
In this paper, we present a set of orchestration extensions to support application-aware adaptation called \emph{\system}. The main observation underlying \system is that container-orchestration platforms allow distributed applications to programmatically drop, redirect, reorder, and transform network data through technologies like sidecar proxies~\cite{envoy} and service-meshes~\cite{istio,linkerd}. \system provides a crisp abstraction on top of these technologies for making decisions about network data using application semantics. 

\system's approach to application-aware adaptation has three advantages. First, exposing network monitoring and control in a single, stateful programming abstraction simplifies application responsibilities. Applications no longer have to internally maintain network metrics and adaptation triggers. Second, \system allows applications to monitor the progress of requests and promptly take application-aware action when they stall. Third, by cleanly separating an application's adaptation logic from its core functionality, \system allows adaptation strategies to be updated and repurposed without inspecting complex sourcecode or deploying new containers.
% \clearpage

\system supports adaptation through a combination of in-network scripting and asynchronous callbacks. Applications register concise scripts to monitor incoming and outgoing message queues and apply application-specific dropping, redirection, reordering, and transformation policies to requests and responses. \system scripts can also interact with other distributed components through a small set of asynchronous remote procedure calls (RPCs). These calls allow an application to set distributed watchpoints and perform heavyweight, in-place transformations like image transcoding. Our case studies in Section~\ref{sec:evaluation} show how applications can benefit from \system.

%\system's in-network processing abstraction allows applications to access network conditions and manipulate HTTP message queues XXX. 

%These two mechanisms work in tandem. Callbacks support adaptation to persistent changes, and in-network processing allows applications to recover from 

This paper makes the following contributions:

\begin{smitemize}
    \item We identify application-aware adaptation as the key to maintaining acceptable service quality under resource scarcity in container-orchestration platforms.
    \item We design and implement a crisp in-network processing abstraction for managing network data with application semantics.
    \item Experiments with our prototype show that (1) by using \system, ML applications at the edge can utilize cloud resources when available and operate without interruption when disconnected, (2) \system enables the Fugu~\cite{yan-nsdi20} video server to eliminate all stalling while sacrificing only 6-24\% mean resolution, and (3) \system adds less than 10\% overhead to the 99th percentile request latency compared to a baseline sidecar.
\end{smitemize}

The rest of the paper is organized as follows. Section~\ref{sec:principles} describes our design principles. Section~\ref{sec:design} describes the \system design. Section~\ref{sec:evaluation} presents an evaluation of our \system prototype. Section~\ref{sec:related} describes related work. And Section~\ref{sec:conclusions} presents our conclusions.


==> text/limit.tex <==
\section{Limitation}
\label{sec:limit}

\system makes tradeoff between application \emph{fidelity} and
\emph{performance}; it has some engineering and principal limitations that are
worthwhile to investigate in the future. First, the \system's script executes
per message received. Though we have not encountered a problem, this can be
problematic for applications that send a new message only after receiving an
ack for old message processed. This limitation may add round-trip latency to
trigger adaptation script. 
\joseph{can we say this is with strict consistency?}
Second, \system is limited to inter-pod transfers; ingress messages to the
cluster or local transfers can benefit further from the principles
incorporated in \system. 
%% Not sure not-dropping-all is principal or artifct
For stream-processing payload, not all messages can be dropped by the
\system's script. This is because the underlying protocol, Netty expects at
least one message arrived. 

%% engineering (artifact) limits
\system does not support WebSocket for video streaming applications. So, new
systems like Fugu~\cite{yan-nsdi20} requires application modifications unless
streams are proxyed to transport over HTTP or Netty. 
Also, \system provides a marginal benefit for newer video format containers
that are not self-descriptive (e.g., fragmented MP4). This is because a client
player fetches metadata only once when it starts. From our limited experience,
the players display broken frames when the \system's script transforms chunks.
To provide significant benefit, \system requires the players to refresh
metadata periodically.

\joseph{TODO: several reviewers point out that it's worth mentioning
adaptations that we consider out of scope or simply, BB can't handle.}

%%
% two types of limitation: artifact (A) and principal (P)

% Video streaming: BB is limited to handle only self-descriptive video chunks
% that embed metadata in the chunks. On the other hands, fragmented MP4 (fMP4)
% format, for instance, initializes the client decoder with specific parameters
% (e.g., bitrate, resolution) prior to receiving actual data chunks. In this
% case, BB’s adaptation scheme that downsamples chunks dynamically doesn’t work.
% \system provides a marginal benefit for fragmented MP4 containers, because
% metadata required for client-side decoder is fetched only once. Chunks are
% streamed without the metadata. In other words, \system giving back a wrong chunk
% breaks the assumption by client player that it has received what it asked for.

% Stream processing: BB is limited to handle inter-pod transfers; ingress and
% local transfers can’t be intercepted by BB. Also, BB assumes application
% developers to write the Lua script because it requires application-specific
% semantics (e.g., JSON) to decide what to do with data intercepted.

% Stream processing-2: BB can’t drop “all” app data at once. This is due to the
% Flink implementation of credit-based flow control, which requires receiving at
% least one app message before polling next batch.

% General: BB’s Lua script is executed per message, which is addressed in the
% paper already. Although we haven’t encountered a problem yet, this can be
% problematic for clients that expected requested message to arrive before
% requesting a new one (e.g., video streaming). In such case, BB can adapt only
% once when the message enters the queue. However, this can be easily solved by
% transmitting periodic sentinel requests to trigger the Lua script.


% Protocol: BB supports only HTTP and Netty protocols. No support for
% WebSocket.
% \system has no support for WebSocket. Thus, new systems like
% Fugu~\cite{yan-nsdi20} requires application modification unless streams are
% proxyed to transport over HTTP.

% Although there have been works that place adaptive
% intelligence at the server instead of the client, the approach requires special
% clients or extensive application modificaiton.



==> text/metrics.tex <==
% BB collects the following network metrics:
% - TCP metrics: congestion window, RTT, sent and acked bytes, in-flight, etc.
%   [list of them: https://linuxgazette.net/136/pfeiffer.html ]
% Below metrics can be measured only if server sends messages first.
% - latency: time diff between request and response.
% - bandwidth: uses latency & size to update weighted estimation.
%    bwest_i = (w * bwest_i-1) + (1 - w) (size / time diff)
%  --> shim layer reports **raw** bw estimation.
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%% original texts from Section 4.3 (In-network scripting)
% To help scripts make good adaptation decisions, \system exports a number of runtime performance metrics. At the lowest level, \system exposes TCP metrics, such as the congestion window size, number of in-flight packets, and mean round trip time (RTT). \system also exposes the average end-to-end latency for messages in a queue, which Envoy calculates using request and response arrival times. In addition, \system provides information about how long each messages has spent in a queue through an object-item's age property. 

% Finally, network bandwidth is a crucial metric for numerous adaptation strategies.  \system does not give scripts information about the available bandwidth along a physical link, but it calculates the observed bandwidth for messages forwarded from particular queue. This allows scripts to reason about the observed bandwidth along their path of interest. For example, scripts can detect that a path has been disconnected if its observed bandwidth drops to zero.


%%%%%%%%%%% detailed texts for Landon
\system retrieves TCP metrics through Linux's socket API, using TCPInfo struct.
\system measures the end-to-end latency and bandwidth through Envoy's tapping
mechanism that tags UID for a request-response pair. When server sends a
request, \system logs a timestamp of the message to compute the end-to-end
latency when receiving the response back from client. \system estimates
bandwidth through three steps. First, it logs the size of request and time
elapsed to send messages from the queue. It detects the messages are fully
transmitted to client by periodically checking TCP's sequence number. Given
Maximum Transmission Unit (MTU) rarely changes, we can compute the exact
sequence number to expect based on the payload size. Finally, given a recent
bandwidth measure, \system updates bandwidth estimation using weighted moving
average. 

%% why couldn't we estimate bandwidth for video streaming and require shim layer?
When client without \system initiates interaction by sending HTTP request,
rather than sever with \system sending HTTP request, the initial message is too
small to estimate bandwidth. Unfortunately, when server responses back with
sufficient payload, \system stateless filter has no access to the corresponding
socket handler after the response leaves a \system's queue. In other words,
Envoy does not actually send out bytes until the full response is flushed from
\system's queue. This was not a problem with the server initiating because Envoy
allows filter to access the socket that waits for response back.


==> text/principles.tex <==
\section{Design principles}
\label{sec:principles}

To provide application-aware adaptation for container orchestration, we designed \system with the following principles in mind.

\noindent \textbf{Separate adaptation logic from the rest of the application.} Application-oblivious responses to resource scarcity can fairly reallocate resources, but only the application knows how to best utilize its allocation. For example, machine-learning (ML) applications can adapt to bandwidth drops by sending lower-quality data to an inference model, and can adapt to increased network latency by sending data to a faster, lower-quality model~\cite{hsieh-osdi18, jiang-sigcom18}. Similarly, video-streaming applications adapt to changing network conditions by trying to dynamically match served bitrates to client bandwidth~\cite{yan-nsdi20}. 

The dominant approach to application-aware adaptation for orchestrated applications is tightly integrating adaptation strategies with the rest of the application logic. For example, consider a video-analytics application that uploads video frames from a camera to an object detector in the cloud. If the application wants to adjust the resolution of its frames to account for decreased bandwidth, it must monitor network conditions, manage bandwidth triggers, and reconfigure how it encode frames. If another developer wants to understand the adaptation strategy or repurpose it for a different ML application, they must inspect and copy the code.

A primary benefit of building applications for orchestrated environments is that distributed applications can be composed of re-usable, self-contained container images. Separating the adaptive logic from the rest of the application reinforces this approach and allows common strategies to be better understood and used in different contexts. For \system, we identify \emph{sidecar proxies} as an ideal place to separate adaptive logic from the rest of an application.
\joseph{didn't show a script is re-usable explicitly? like using video streaming script with both HLS and DASH?} 

\noindent \textbf{Present a message-queue abstraction to in-network computations.}
%Sidecars are transparent, user-level network proxies that interpose on all application communication. The most popular sidecar is Envoy~\cite{envoy}, which supports in-network processing via \emph{filters}.
% Filters are small, stateless code snippets that operate on individual messages. Filters have full access to a message and can perform simple operations, such as redirection, dropping, and payload transformation.
%Developers commonly use Envoy filters for monitoring and traffic shaping, such as collecting telemetry, load-balancing, and performing A/B testing. 
%Envoy supports filters at several layers of the network stack, including HTTP. 
Unfortunately, Envoy's stateless, per-message approach is a poor fit for many of the adaptation strategies we would like to support. In particular, applications with realtime or near-realtime constraints, like video analytics and video streaming, benefit from adapting to message stalls. For example, if a video frame destined for an object-detection model appears likely to miss its deadline, a video-analytics application could drop the message, reduce its resolution, or redirect it to a different model. This kind of reasoning is not possible within Envoy because its filters only process messages as they arrive, which is rarely the moment when adaptive action is required.

As a result, \system presents a message-queue abstraction to in-network computations. Message queues give in-network computations access to information about messages' order and provide a natural way to expose information that changes over time, such as a message's age. In addition, dropping, redirecting, reordering, and transforming network data are easy to map onto a small number of message-queue operations.
\shadi{is this point really a design goal? it seems out of place a bit.}


%\noindent \textbf{Meet developers where they are.} Finally, orchestration platforms make extensive use of declarative languages like YAML, and many developers are comfortable with other declarative languages like SQL. When deciding how to programmatically present message queues in \system, we initially considered a declarative interface. However, nearly all adaptation strategies of which we are aware are implemented in imperative languages. Giving \system a declarative interface would have not only asked developers to reimplement their strategies in a new language, but it would also have asked them to re-conceptualize those strategies in an unfamiliar style. Thus, \system provides a simple imperative scripting environment for implementing application-aware adaptation.

\shadiC{

\noindent \textbf{A simple and low-overhead adaptation API.} Building adaptation logic should not impose huge burdens on the developers. Ideally, developers should be able to express their adaptation logic with tens of lines of code in a familiar style. Also, they should be able to easily tailor their adaptation logic for new deployment environments, e.g., rural vs urban areas.  Thus, \system provides a simple imperative scripting environment for implementing application-aware adaptation.

Moreover, the Envoy sidecar is a shared resource on the critical path, so any mechanism must be lightweight, deterministic, and focused on control plane actions. Any data-centric work was to be done via external, asynchronous means. 



	
%When designing \system{'s} adaptation API, we two main goals in mind:
%\squishlist
%\item \textit{Simplicity:} Building adaptation logic should not impose huge burdens on the developers to build adaption logic. Ideally, developers should be able to express their adaptation logic with tens of lines of code. Also, they should be able to easily tailor their adaptation logic for new deployment environments, e.g., rural vs urban areas.
%\item \textit{Low overhead on the critical path:} The Envoy sidecar is a shared resource on the critical path, so any mechanism must be lightweight, deterministic, and focused on control plane actions. Any data-centric work was to be done via external, asynchronous means.
%\squishend
%
%\shadi{maybe these goals should moved earlier on?}
%
%This motivated a few key decisions. We first
%explored declarative interfaces like YAML or SQL, but decided it had too much unnecessary functionality that could be a runtime
%liability, while simple things were too complicated to express. This motivated a shift from
%declarative SQL to imperative Lua. Furthermore, we explicitly do not support the use of Lua
%libraries beyond the standard, built-in set, keeping in-script behavior simple, low overhead, and less prone to security attacks.

}

